Cross-layer Path Selection in Multi-path Transport Protocol for Mobile Devices

MPTCP is a new transport protocol that enables mobile devices to use multiple physical paths simultaneously through several network interfaces, such as WiFi and Cellular. However, wireless path capacities change frequently in the mobile environments, causing challenges for path selection. For example, WiFi associated paths often become poor as devices walk away, since WiFi has intermittent connectivity caused by the short signal coverage and stochastic interference. MPTCP's native decision based on hysteretic TCP-layer estimation will miss the real switching point of wireless quality, which may cumulate packets on the broken path and causes serious packets reinjection. Through analyzing a unique dataset in the wild, we quantitatively study the impact of MAC-layer factors on the aggregated performance of MPTCP. We then propose a decision tree approach for cross-layer path selection that decides which path to carry the incoming packets dynamically according to the prior learned schemes. A prototype of the path selection system named SmartPS, which proactively probes the wireless environments, is realized and deployed in Linux and Android. Evaluation results demonstrate that our SmartPS can efficiently utilize the faster path, with goodput improvements of up to 29%.

==> ack.tex <==
%!TEX root = main.tex

\section*{Acknowledgments}

This work was supported by the National Natural Science Foundation of China  No. 61572475 and 61502460, the National High-tech R\&D Program of China No. 2015AA010201, the Beijing Natural Science Foundation No. 4162057.



==> adapt.tex <==
%!TEX root = main.tex

\section{Adapting Decision Tree Algorithm}
\label{sec:adapt}
\subsection{Partitioning Basis}

==> back <==
Table 1 illustrates the performance comparison of the same MPTCP connection except for a different path selection decision: $LTE\_First$ (LF) or $WiFi\_First$ (WF). We label.
\begin{table}[h]
\scriptsize
\centering
\caption{results of the circular opening angles}
\label{Tab01}
\begin{tabular}{cccccc}
\toprule
\multicolumn{2}{c}{Application Goodput (Mbps)} & \multicolumn{2}{c}{Application Delay (ms)} & \multirow{2}{*}{Better Decision}		\\
\cmidrule(r){1-2} \cmidrule(r){3-4}
$LF$		&$WF$		&$LF$		&$WF$		\\
\midrule
15.4		&23.2		&45.3		&30.6		&$WF$		\\
21.5		&18.7		&37.1		&42.3		&$LF$		\\
15.3		&15.3		&30.3		&26.2		&$WF$		\\
21.4		&21.4		&27.5		&34.4		&$LF$		\\
\bottomrule
\end{tabular}
\end{table}



\begin{table*}[ht]
\scriptsize
\centering
\caption{results of the circular opening angles}
\label{Tab02}
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{4}{c}{WiFi} & \multicolumn{5}{c}{LTE} & \multirow{2}{*}{Label}		\\
\cmidrule(r){1-4} \cmidrule(r){5-9}
$RTT$	&$RSSI$	&$CWND$	&$FQ$	&$RTT$	&$RSSI$	&$SINR$	&$CWND$	&$FQ$	\\
\midrule
52		&-30		&15		&2.4		&63	&-45		&21		&12		&3	&$WiFi\_First$	\\
69		&-80		&4		&5		&48	&-23		&28		&25		&5	&$LTE\_First$ \\
46		&-45		&19		&2.4		&54	&-57		&18		&11		&4	&$WiFi\_First$	\\
%21.4		&21.4		&27.5		&34.4		&$LF$	&23.2		&45.3		&30.6		&$WF$	\\
\bottomrule
\end{tabular}
\end{table*}


Preliminary experiment in section has confirmed the qualitative result that RSSI have the . We futher largest values of absolute Kendall coefficient [14], which is a measure of correlation without assumptions. When applied to further path selection approach, MAC-layer attributes can be collected during the probing step of a Mobile device before its authentication and association. 


%MPTCP连接的性能由底层的TCP子流决定。而在无线网络中，第一跳网络的质量尤为重要。调度器的设计中说明很多TCP层的参数都影响MPTCP的整体性能，RTT是最主要的因素。仅使用RTT做路径选择主要包含以下两个原因，为了简单化。选择意味着对比，但是当比较的因素过多时，无法确定那个因素应该最先对比。信息熵通过熵增原理，从开始决策价值最大。我们只需要将关联起来。但是数据越完备，数据足够多除了RTT，有很多TCP层的性能参数可以用来做路径选择，但是为何没有融合到一起进行路径选择呢？由于不是线性模型，无法通过简单的阈值来进行判断。

%一个物理接口是被很多不同的共享的，但是一个MPTCP子流通常只建立一条子流。因此，我们可以将TCP子流用其接口名对应。有很多衡量TCP子流的度量，而且是统一的，如：选择一个子流需要根据历史的信息，RTT，丢包率，不能应对当前的无线网络的状态。但是，物理层的信息不统一，RSSI, SINR, 2.4Ghz/5Ghz 

%不需要计算相关系数，由于后面决策树建立的时候，信息熵会计算出谁对决策结果的影响最大。

%delivery latency, 由于网络的异构性, 乱序导致，定性的探索，后面需要定量的探索。作出一个决策需要大量的数据，显然定性的方式无法帮助我们做决策。我们首先探讨，物理信号的影响，之后探讨minrtt,图中显示 MinRTT错过最佳的切换点。head-of-line blocking, . 物理信号在MPTCP已经应用过很多次，设置没有经验的阈值。一个确定的数学模型，需要通过大量的数据训练出来。

